Video-Panda: Parameter-efficient Alignment for Encoder-free Video-Language Models

We present an efficient encoder-free approach for video-language understanding that achieves competitive performance while significantly reducing computational overhead. Current video-language models typically rely on heavyweight image encoders (300M-1.1B parameters) or video encoders (1B-1.4B parameters), creating a substantial computational burden when processing multi-frame videos. Our method introduces a novel Spatio-Temporal Alignment Block (STAB) that directly processes video inputs without requiring pre-trained encoders while using only 45M parameters for visual processing - at least a 6.5$\times$ reduction compared to traditional approaches. The STAB architecture combines Local Spatio-Temporal Encoding for fine-grained feature extraction, efficient spatial downsampling through learned attention and separate mechanisms for modeling frame-level and video-level relationships. Our model achieves comparable or superior performance to encoder-based approaches for open-ended video question answering on standard benchmarks. The fine-grained video question-answering evaluation demonstrates our model's effectiveness, outperforming the encoder-based approaches Video-ChatGPT and Video-LLaVA in key aspects like correctness and temporal understanding. Extensive ablation studies validate our architectural choices and demonstrate the effectiveness of our spatio-temporal modeling approach while achieving 3-4$\times$ faster processing speeds than previous methods. Code is available at https://jh-yi.github.io/Video-Panda.

==> tables/5_resolution.tex <==
\begin{table}[t]
   \centering
   \resizebox{.5\textwidth}{!}{
       \begin{tabular}{cccc}
           \toprule
           \textbf{Resolution} & \textbf{Resolution} & \textbf{MSVD-QA} & \textbf{Activity Net-QA} \\
           \midrule
           Video-Panda (LR) & $224^2$ & 52.5/3.4 & 36.1/3.2 \\
           Video-Panda & $448^2$ & 64.7/3.8 & 40.0/3.3 \\
           Video-Panda (HD-overflow) & $896^2$ & 57.9/3.6 & 37.8/3.2 \\
           Video-Panda (HD-fitu) & $896^2$ & 60.1/3.6 & 38.5/3.2 \\
           Video-Panda (HD-LSD4x4) & $896^2$ & 61.8/3.7 & 39.3/3.2 \\
           TODO Res. + larger context length & & & \\
           
           \bottomrule
       \end{tabular}
   }
   \caption{Ablation study on video resolution.   }
   \label{tab:ablation_resolution}
\end{table}

==> tables/r_flops.tex <==
\begin{table}[!t]
\hfill
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            \textbf{Model} & \textbf{Vision Size (M)} & \textbf{FLOPs (G)} & \textbf{Latency (ms)}\\
            \midrule
            Video-ChatGPT & 307 & 8109.1 & 171\\
            Video-LLaVA & 425 & 864.1 & 125 \\
            \midrule
            Video-Panda & 45 & 105.5 & 41\\
            \bottomrule
        \end{tabular}
    }
    \caption{Params/FLOPs/Latency comparison of the visual part.}
    \label{tab:complexity}
\end{table}


